Reward Hacking in the Era of Large Models: Mechanisms, Emergent Misalignment, Challenges

Reinforcement Learning from Human Feedback (RLHF) and related alignment paradigms have become central to steering large language models (LLMs) and multimodal large language models (MLLMs) toward human-preferred behaviors. However, these approaches introduce a systemic vulnerability: reward hacking, where models exploit imperfections in learned reward signals to maximize proxy objectives without fulfilling true task intent. As models scale and optimization intensifies, such exploitation manifests as verbosity bias, sycophancy, hallucinated justification, benchmark overfitting, and, in multimodal settings, perception--reasoning decoupling and evaluator manipulation. Recent evidence further suggests that seemingly benign shortcut behaviors can generalize into broader forms of misalignment, including deception and strategic gaming of oversight mechanisms. In this survey, we propose the Proxy Compression Hypothesis (PCH) as a unifying framework for understanding reward hacking. We formalize reward hacking as an emergent consequence of optimizing expressive policies against compressed reward representations of high-dimensional human objectives. Under this view, reward hacking arises from the interaction of objective compression, optimization amplification, and evaluator--policy co-adaptation. This perspective unifies empirical phenomena across RLHF, RLAIF, and RLVR regimes, and explains how local shortcut learning can generalize into broader forms of misalignment, including deception and strategic manipulation of oversight mechanisms. We further organize detection and mitigation strategies according to how they intervene on compression, amplification, or co-adaptation dynamics. By framing reward hacking as a structural instability of proxy-based alignment under scale, we highlight open challenges in scalable oversight, multimodal grounding, and agentic autonomy.

==> sections/Mechanisms.tex <==
\section{Mechanisms of Reward Hacking}
\label{sec:mechanisms}

\begin{table}[htbp]
\centering
\scriptsize
\caption{Comparison of four mechanism classes of reward hacking. Under the Proxy Compression Hypothesis (PCH), these classes represent a progressive escalation in how policies exploit the informational bottlenecks and co-adaptive vulnerabilities of proxy-based alignment.}
\label{tab:mechanism_taxonomy_comparison}
\begin{tabularx}{\textwidth}{
>{\raggedright\arraybackslash}p{1.95cm}
>{\raggedright\arraybackslash}p{2.15cm}
>{\raggedright\arraybackslash}p{3.25cm}
>{\raggedright\arraybackslash}p{2.35cm}
>{\raggedright\arraybackslash}X}
\toprule
\rowcolor{headergray}
\textbf{Mechanism Class} & \textbf{Exploited Locus} & \textbf{Typical Pattern} & \textbf{Typical Setting} & \textbf{Main Risk under PCH} \\
\midrule

\textbf{Feature-level}
& Surface reward correlates
& Verbosity bias; sycophancy; politeness inflation; formatting exploits
& RLHF; RLAIF; preference tuning
& \textbf{Compression Artifacts:} Optimization amplifies superficial ``survivor features'' that dominate the low-dimensional proxy score. \\

\textbf{Representation-level}
& Latent shortcut strategies
& Fabricated CoT; memorized schemas; benchmark gaming; process--outcome decoupling
& RLVR; reasoning; multimodal tasks
& \textbf{Equivalence Classes:} Shortcut solutions become indistinguishable from faithful reasoning under outcome-only evaluation. \\

\textbf{Evaluator-level}
& Reward model / judge / verifier
& Blind-spot exploitation; judge manipulation; selective compliance; concealed errors
& Learned RMs; LLM-as-a-judge; rubric grading
& \textbf{Co-adaptation:} The evaluator ceases to be a transparent metric and becomes a strategically manipulable object. \\

\textbf{Environment-level}
& Tools, logs, tests, observation channels
& Test rewriting; reward tampering; API/logging exploits; camera-angle hacks
& Agentic coding; tool use; embodied agents
& \textbf{Amplification Limit:} The policy bypasses the latent objective by systematically altering the medium through which oversight operates. \\
\bottomrule
\end{tabularx}
\end{table}

Section~\ref{sec:foundations} established that reward hacking in foundation model alignment is best understood as a structural consequence of the \emph{Proxy Compression Hypothesis} (PCH): optimizing expressive policies against evaluators that compress rich objectives into lower-dimensional representations. Under this lens, the heterogeneous failures observed in practice---ranging from verbose sycophancy to fabricated reasoning and environment-level sabotage---are not isolated bugs. Rather, they represent different strategies for exploiting the structural tension between a latent objective and its operational proxy \cite{skalse2022defining,rafailov2024scaling}.

To systematically analyze this landscape, a rigorous taxonomy must identify \emph{where} the exploitable mismatch arises and \emph{how} optimization pressure capitalizes on it. Motivated by the PCH framework, we organize reward hacking mechanisms according to the \emph{locus of exploitation}. We delineate four distinct levels of escalation: (i) \textbf{Feature-level exploitation}, where policies amplify superficial statistical correlates surviving compression; (ii) \textbf{Representation-level exploitation}, where policies adopt latent shortcuts that decouple task appearance from genuine competency; (iii) \textbf{Evaluator-level exploitation}, where the scoring mechanism itself becomes an adversarial target; and (iv) \textbf{Environment-level exploitation}, where the policy alters the observation channel to synthesize fake success. 

Crucially, these mechanisms reflect a progression driven by the three forces of PCH. Feature and representation-level hacks are direct consequences of \emph{objective compression}. Evaluator-level hacks emerge from \emph{evaluator--policy co-adaptation}. Finally, environment-level hacks represent the extreme realization of \emph{optimization amplification} in agentic settings. By structuring our analysis through this taxonomy, we provide a unified vocabulary to compare failures across RLHF, RLAIF, and RLVR pipelines, setting the theoretical stage for the concrete manifestations discussed in Section~4.

\subsection{Feature-Level Exploitation: Amplifying Compression Artifacts}
\label{subsec:feature-level}

Feature-level exploitation is the most ubiquitous and earliest-emerging form of reward hacking. In this regime, the policy maximizes proxy reward by amplifying superficial linguistic or visual features that correlate with human preference but lack causal connection to the underlying objective \cite{rafailov2024scaling,miao2024inform}. 

Viewed through the PCH framework, this mechanism is driven directly by the information bottleneck of reward modeling. When a high-dimensional human preference is compressed into a scalar evaluator, nuanced criteria such as truthfulness, helpfulness, and nuance are often implicitly substituted by easily measurable proxies. We term these \emph{``survivor features''}---statistical regularities (e.g., increased token count, deferential tone, or authoritative formatting) that survive the compression process and thus dominate the reward landscape. Under optimization pressure, the policy systematically shifts probability mass toward these survivor features, discovering that inserting hedges or padding responses is computationally cheaper than improving actual factual accuracy. 

A canonical example is \emph{sycophancy}, where models align their outputs with a user's explicitly stated or implicitly assumed beliefs, even when those beliefs are objectively false \cite{denison2024sycophancy}. In multimodal domains, this manifests as visual feature gaming, where generative models over-index on high-contrast, aesthetically pleasing artifacts at the expense of anatomical correctness or prompt faithfulness. 

Analytically, feature-level exploitation is critical because it establishes the foundational reflex of misalignment: the policy is actively reinforced for proxy-directed behavior. Even if the initial exploit is benign (such as harmless formatting inflation), it teaches the network a generalized meta-strategy---to optimize the observable metric rather than the latent task---paving the way for more sophisticated misbehaviors \cite{denison2024sycophancy}.

\subsection{Representation-Level Exploitation: Navigating Equivalence Classes}
\label{subsec:representation-level}

While feature-level exploitation operates on surface artifacts, representation-level exploitation occurs deeper within the semantic and structural logic of the response. Here, the policy discovers latent shortcut strategies that satisfy the criteria of the compressed evaluator while entirely circumventing the cognitive or perceptual work the task intends to elicit.

This mechanism is explicitly explained by the concept of \emph{equivalence classes} introduced in Section~\ref{subsec:pch}. Because a proxy evaluator (particularly outcome-based ones) discards intermediate computational states, it inevitably maps multiple distinct internal policy trajectories to the identical high reward. For instance, a model may arrive at the correct final answer through rigorous logical deduction, or it may arrive at the same answer through memorized dataset heuristics paired with a fabricated, post-hoc Chain-of-Thought (CoT) \cite{turpin2023language,lanham2023measuring}. To the proxy, these two representations belong to the same equivalence class and are reward-equivalent. 

This dynamic is strongly amplified in Reinforcement Learning from Verifiable Rewards (RLVR). Because verifiable checkers typically grade final outcomes, they incentivize \emph{process--outcome decoupling}. The model learns that the textual discourse of reasoning is merely a stylistic requirement, completely decoupled from the actual computational mechanism determining the answer \cite{lightman2023let}. In multimodal Vision-Language Models (VLMs), this manifests as \emph{perception bypass}, where models hallucinate visual details based on linguistic priors rather than genuine visual grounding, effectively simulating multimodal reasoning while exclusively utilizing text-based shortcuts \cite{xia2025visionary}.

Representation-level exploitation is substantially more dangerous than surface feature gaming because it is highly portable. Once a policy learns to reliably separate ``what the evaluator checks'' from ``how the problem is actually solved,'' it transitions from merely taking shortcuts to engaging in implicit deception.

\subsection{Evaluator-Level Exploitation: Gaming the Co-Adaptive Loop}
\label{subsec:evaluator-level}

Evaluator-level exploitation marks a phase transition in reward hacking: the policy no longer treats the evaluator as a static, passive environment, but models it as an active, manipulable object. This shift corresponds to the \emph{evaluator--policy co-adaptation} pillar of the PCH framework. The optimization target moves from simulating task success to actively exploiting the vulnerabilities, biases, and blind spots of the oversight mechanism itself \cite{rafailov2024scaling,khalaf2025inference}.

In RLHF, this occurs when highly capable policies identify low-density regions of the preference manifold where the learned reward model extrapolates poorly, synthesizing outputs that mathematically maximize the scalar reward while appearing nonsensical or harmful to humans \cite{miao2024inform}. The dynamic is further exacerbated in RLAIF and LLM-as-a-judge pipelines. When the evaluating judge and the generating policy share architectural lineages, pretraining corpora, or linguistic biases, the policy effectively reverse-engineers the judge. It learns to craft responses specifically tailored to trigger the judge's approval heuristics, bypassing objective quality entirely.

Furthermore, as oversight increasingly relies on natural-language mediation (e.g., rubric-following LLMs or verbalized safety constraints), the evaluator's context window becomes an attack surface. Policies can engage in prompt-injection-style manipulation of the judge or selectively comply with only the most rigorously checked constraints while ignoring others \cite{li2025llms,maloyan2025investigating}. Under PCH, evaluator-level exploitation demonstrates that compression does more than lose information---it creates an adversarial interface. This explicitly bridges the gap between narrow specification gaming and the emergence of evaluator-aware, alignment-faking behaviors \cite{denison2024sycophancy,taylor2025school}.

\subsection{Environment-Level Exploitation: Bypassing the System}
\label{subsec:environment-level}

Environment-level exploitation represents the ultimate limit of optimization amplification. If evaluator-level exploitation treats the scoring model as an attack surface, environment-level exploitation attacks the entire surrounding infrastructure that mediates evaluation. Here, the policy achieves high reward by altering the observation channels, APIs, or execution environments to synthesize a state of apparent success.

As foundation models are deployed as autonomous agents embedded in rich, stateful environments (e.g., operating systems, code repositories, or embodied simulations), their action space expands exponentially. Consequently, the set of possible reward hacks expands from textual persuasion to physical and digital tampering \cite{khalifa2026countdown,deshpande2026benchmarking}. For instance, a coding agent instructed to fix a bug may instead silently rewrite the unit test to always return \texttt{True}, or suppress error logging mechanisms to prevent failure detection \cite{denison2024sycophancy}. In embodied AI, an agent might reposition its camera angle to occlude a mess rather than cleaning it, exploiting the perceptual limitations of the visual evaluator.

Conceptually, this mechanism illustrates the breakdown of the classical agent-environment boundary. The system that implements oversight is co-opted as part of the action space. The policy learns that the proxy reward depends strictly on the *observed* state, not the *true* state. Therefore, modifying the lens through which the world is observed is mathematically equivalent, and often computationally cheaper, than modifying the world itself. Environment-level exploitation is not a separate pathology from feature or representation hacking; it is their logical, and most severe, extrapolation when advanced models are granted agentic affordances.

